Piano Skills Assessment

Can a computer determine a piano player's skill level? Is it preferable to base this assessment on visual analysis of the player's performance or should we trust our ears over our eyes? Since current CNNs have difficulty processing long video videos, how can shorter clips be sampled to best reflect the players skill level? In this work, we collect and release a first-of-its-kind dataset for multimodal skill assessment focusing on assessing piano player's skill level, answer the asked questions, initiate work in automated evaluation of piano playing skills and provide baselines for future work. Dataset is available from: https://github.com/ParitoshParmar/Piano-Skills-Assessment.

==> Sections/Related.tex <==
\section{Related Work}

\textbf{Piano + Computer Vision:} There has been work exploring the use of computer vision in determining the accuracy of pianists \cite{lee2019observing}; automatic transcription \cite{li2018creating, koepke2020sight, li2020robust}; generating audio from video/silent performance \cite{kang2019virtual, su2020audeo, gan2020foley}; or generating pianist's body pose from audio/MIDI \cite{li2018skeleton}. However, there has been no work addressing the prediction of pianist's skill level from the recording of their performance. Our work is the first to address prediction of pianist's skill level. 

\noindent\textbf{Skills-Assessment/Action Quality Assessment:} While there has been quite some progress recently in the areas of SA \cite{doughty2019pros, li2019manipulation, wang2020towards} and AQA \cite{li2018end, xiang2018s3d, li2018scoringnet, xu2019learning, parmar2019hallucinet, sardari2019view, pan2019action, mtlaqa, wang2020hands, tang2020uncertainty}, none of these works address assessment of pianist's skills. Moreover, ours is the first work to explore a multimodal learning approach in skills-assessment or action quality assessment.

==> refs_all.tex <==
@inproceedings{imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}

@inproceedings{resnet,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@incollection{pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
pages = {8026--8037},
year = {2019},
}

@inproceedings{librosa,
  title={librosa: Audio and Music Signal Analysis in Python},
  author={McFee,, B. and Raffel,, C. and Liang,, D. and Ellis,, D.P.W. and McVicar,, M. and Battenberg,, E. and Nieto,, O.},
  booktitle = {14th annual Scientific Computing with Python conference},
  series={SciPy},
  month={July},
  doi={https://doi.org/10.25080/Majora-7b98e3ed-003},
  year={2015}
}

@article{adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{ucf101,
  title={UCF101: A dataset of 101 human actions classes from videos in the wild},
  author={Soomro, Khurram and Zamir, Amir Roshan and Shah, Mubarak},
  journal={arXiv preprint arXiv:1212.0402},
  year={2012}
}

@inproceedings{lee2019observing,
  title={Observing pianist accuracy and form with computer vision},
  author={Lee, Jangwon and Doosti, Bardia and Gu, Yupeng and Cartledge, David and Crandall, David and Raphael, Christopher},
  booktitle={2019 IEEE Winter Conference on Applications of Computer Vision (WACV)},
  pages={1505--1513},
  year={2019},
  organization={IEEE}
}

@article{suteparuk2014detection,
  title={Detection of piano keys pressed in video},
  author={Suteparuk, Potcharapol}
}

@inproceedings{oka2013marker,
  title={Marker-less piano fingering recognition using sequential depth images},
  author={Oka, Akiya and Hashimoto, Manabu},
  booktitle={The 19th Korea-Japan Joint Workshop on Frontiers of Computer Vision},
  pages={1--4},
  year={2013},
  organization={IEEE}
}

@inproceedings{gorodnichy2006detection,
  title={Detection and tracking of pianist hands and fingers},
  author={Gorodnichy, Dmitry O and Yogeswaran, Arjun},
  booktitle={The 3rd Canadian Conference on Computer and Robot Vision (CRV'06)},
  pages={63--63},
  year={2006},
  organization={IEEE}
}

@inproceedings{takegawa2006design,
  title={Design and implementation of a real-time fingering detection system for piano performance},
  author={Takegawa, Yoshinari and Terada, Tsutomu and Nishio, Shojiro}
}

@article{li2018creating,
  title={Creating a multitrack classical music performance dataset for multimodal music analysis: Challenges, insights, and applications},
  author={Li, Bochen and Liu, Xinzhao and Dinesh, Karthik and Duan, Zhiyao and Sharma, Gaurav},
  journal={IEEE Transactions on Multimedia},
  volume={21},
  number={2},
  pages={522--535},
  year={2018},
  publisher={IEEE}
}

@inproceedings{deb2016image,
  title={An image analysis approach for transcription of music played on keyboard-like instruments},
  author={Deb, Souvik Sinha and Rajwade, Ajit},
  booktitle={Proceedings of the Tenth Indian Conference on Computer Vision, Graphics and Image Processing},
  pages={1--6},
  year={2016}
}

@article{akbari2015real,
  title={Real-time piano music transcription based on computer vision},
  author={Akbari, Mohammad and Cheng, Howard},
  journal={IEEE Transactions on Multimedia},
  volume={17},
  number={12},
  pages={2113--2121},
  year={2015},
  publisher={IEEE}
}

@inproceedings{koepke2020sight,
  title={Sight to Sound: An End-to-End Approach for Visual Piano Transcription},
  author={Koepke, A Sophia and Wiles, Olivia and Moses, Yael and Zisserman, Andrew},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1838--1842},
  year={2020},
  organization={IEEE}
}

@inproceedings{li2020robust,
  title={Robust Piano Music Transcription Based on Computer Vision},
  author={Li, Jun and Xu, Wei and Cao, Yong and Liu, Wei and Cheng, Wenqing},
  booktitle={Proceedings of the 2020 4th High Performance Computing and Cluster Technologies Conference \& 2020 3rd International Conference on Big Data and Artificial Intelligence},
  pages={92--97},
  year={2020}
}

@article{su2020audeo,
  title={Audeo: Audio generation for a silent performance video},
  author={Su, Kun and Liu, Xiulong and Shlizerman, Eli},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}

@article{gan2020foley,
  title={Foley Music: Learning to Generate Music from Videos},
  author={Gan, Chuang and Huang, Deng and Chen, Peihao and Tenenbaum, Joshua B and Torralba, Antonio},
  journal={arXiv preprint arXiv:2007.10984},
  year={2020}
}

@article{kang2019virtual,
  title={Virtual Piano using Computer Vision},
  author={Kang, Seongjae and Kim, Jaeyoon and Yoon, Sung-eui},
  journal={arXiv preprint arXiv:1910.12539},
  year={2019}
}


@inproceedings{li2018skeleton,
  title={Skeleton Plays Piano: Online Generation of Pianist Body Movements from MIDI Performance.},
  author={Li, Bochen and Maezawa, Akira and Duan, Zhiyao},
  booktitle={ISMIR},
  pages={218--224},
  year={2018}
}




@COMMENT SKILLS ASSESSMENT
@inproceedings{doughty2018s,
  title={Who's better? who's best? pairwise deep ranking for skill determination},
  author={Doughty, Hazel and Damen, Dima and Mayol-Cuevas, Walterio},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6057--6066},
  year={2018}
}

@inproceedings{doughty2019pros,
  title={The pros and cons: Rank-aware temporal attention for skill determination in long videos},
  author={Doughty, Hazel and Mayol-Cuevas, Walterio and Damen, Dima},
  booktitle={proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7862--7871},
  year={2019}
}

@inproceedings{li2019manipulation,
  title={Manipulation-skill assessment from videos with spatial attention network},
  author={Li, Zhenqiang and Huang, Yifei and Cai, Minjie and Sato, Yoichi},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision Workshops},
  pages={0--0},
  year={2019}
}

@inproceedings{wang2020towards,
  title={Towards Accurate and Interpretable Surgical Skill Assessment: A Video-Based Method Incorporating Recognized Surgical Gestures and Skill Levels},
  author={Wang, Tianyu and Wang, Yijie and Li, Mian},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={668--678},
  year={2020},
  organization={Springer}
}

@article{chen2020toward,
  title={Toward Adaptive Guidance: Modeling the Variety of User Behaviors in Continuous-Skill-Improving Experiences of Machine Operation Tasks},
  author={Chen, Long-fei and Nakamura, Yuichi and Kondo, Kazuaki},
  journal={arXiv preprint arXiv:2003.03025},
  year={2020}
}

@inproceedings{seo2019understanding,
  title={Understanding Sprinting Motion Skills using Unsupervised Learning for Stepwise Skill Improvements of Running Motion.},
  author={Seo, Chanjin and Sabanai, Masato and Ogata, Hiroyuki and Ohya, Jun},
  booktitle={ICPRAM},
  pages={467--475},
  year={2019}
}

@article{li2019automated,
  title={Automated Fine Motor Evaluation for Developmental Coordination Disorder},
  author={Li, Ruimin and Fu, Hong and Zheng, Yang and Lo, Wai-Lun and Jane, J Yu and Sit, Cindy HP and Chi, Zheru and Song, Zongxi and Wen, Desheng},
  journal={IEEE Transactions on Neural Systems and Rehabilitation Engineering},
  volume={27},
  number={5},
  pages={963--973},
  year={2019},
  publisher={IEEE}
}

@article{li2018evaluation,
  title={Evaluation of the fine motor skills of children with DCD using the digitalised visual-motor tracking system},
  author={Li, Ruimin and Li, Bin and Zhang, Shixiong and Fu, Hong and Lo, Wai-Lun and Yu, Jie and Sit, Cindy HP and Wen, Desheng},
  journal={The Journal of Engineering},
  volume={2018},
  number={2},
  pages={123--129},
  year={2018},
  publisher={IET}
}






@COMMENT AQA
@inproceedings{gordon1995automated,
  title={Automated video assessment of human performance},
  author={Gordon, Andrew S},
  booktitle={Proceedings of AI-ED},
  pages={16--19},
  year={1995}
}

@inproceedings{pirsiavash2014assessing,
  title={Assessing the quality of actions},
  author={Pirsiavash, Hamed and Vondrick, Carl and Torralba, Antonio},
  booktitle={European Conference on Computer Vision},
  pages={556--571},
  year={2014},
  organization={Springer}
}

@inproceedings{parmar2016measuring,
  title={Measuring the quality of exercises},
  author={Parmar, Paritosh and Morris, Brendan Tran},
  booktitle={2016 38th Annual International Conference of the IEEE Engineering in Medicine and Biology Society (EMBC)},
  pages={2241--2244},
  year={2016},
  organization={IEEE}
}

@article{xu2019learning,
  title={Learning to score figure skating sport videos},
  author={Xu, Chengming and Fu, Yanwei and Zhang, Bing and Chen, Zitian and Jiang, Yu-Gang and Xue, Xiangyang},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  year={2019},
  publisher={IEEE}
}

@inproceedings{parmar2019action,
  title={Action quality assessment across multiple actions},
  author={Parmar, Paritosh and Morris, Brendan},
  booktitle={2019 IEEE Winter Conference on Applications of Computer Vision (WACV)},
  pages={1468--1476},
  year={2019},
  organization={IEEE}
}

@article{lei2020learning,
  title={Learning effective skeletal representations on RGB video for fine-grained human action quality assessment},
  author={Lei, Qing and Zhang, Hong-Bo and Du, Ji-Xiang and Hsiao, Tsung-Chih and Chen, Chih-Cheng},
  journal={Electronics},
  volume={9},
  number={4},
  pages={568},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{parmar2019hallucinet,
  title={HalluciNet-ing Spatiotemporal Representations Using 2D-CNN},
  author={Parmar, Paritosh and Morris, Brendan},
  journal={arXiv preprint arXiv:1912.04430},
  year={2019}
}

@inproceedings{li2018scoringnet,
  title={ScoringNet: Learning Key Fragment for Action Quality Assessment with Ranking Loss in Skilled Sports},
  author={Li, Yongjun and Chai, Xiujuan and Chen, Xilin},
  booktitle={Asian Conference on Computer Vision},
  pages={149--164},
  year={2018},
  organization={Springer}
}

@article{parsa2020multi,
  title={A Multi-Task Learning Approach for Human Action Detection and Ergonomics Risk Assessment},
  author={Parsa, Behnoosh and Banerjee, Ashis G},
  journal={arXiv preprint arXiv:2008.03014},
  year={2020}
}

@inproceedings{sardari2019view,
  title={View-invariant Pose Analysis for Human Movement Assessment from RGB Data},
  author={Sardari, Faegheh and Paiement, Adeline and Mirmehdi, Majid},
  booktitle={International Conference on Image Analysis and Processing},
  pages={237--248},
  year={2019},
  organization={Springer}
}

@inproceedings{pan2019action,
  title={Action assessment by joint relation graphs},
  author={Pan, Jia-Hui and Gao, Jibin and Zheng, Wei-Shi},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={6331--6340},
  year={2019}
}

@inproceedings{li2018end,
  title={End-to-end learning for action quality assessment},
  author={Li, Yongjun and Chai, Xiujuan and Chen, Xilin},
  booktitle={Pacific Rim Conference on Multimedia},
  pages={125--134},
  year={2018},
  organization={Springer}
}

@inproceedings{xiang2018s3d,
  title={S3d: Stacking segmental p3d for action quality assessment},
  author={Xiang, Xiang and Tian, Ye and Reiter, Austin and Hager, Gregory D and Tran, Trac D},
  booktitle={2018 25th IEEE International Conference on Image Processing (ICIP)},
  pages={928--932},
  year={2018},
  organization={IEEE}
}

@inproceedings{mtlaqa,
  title={What and how well you performed? A multitask learning approach to action quality assessment},
  author={Parmar, Paritosh and Morris, Brendan Tran},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={304--313},
  year={2019}
}

@inproceedings{gao2020asymmetric,
  title={An Asymmetric Modeling for Action Assessment},
  author={Gao, Jibin and Zheng, Wei-Shi and Pan, Jia-Hui and Gao, Chengying and Wang, Yaowei and Zeng, Wei and Lai, Jianhuang},
  booktitle={European Conference on Computer Vision},
  pages={222--238},
  year={2020},
  organization={Springer}
}

@inproceedings{wang2020hands,
  title={Towards a data-driven method for RGB video-based hand action quality assessment in real time},
  author={Wang, Tianyu and Jin, Minhao and Wang, Jingying and Wang, Yijie and Li, Mian},
  booktitle={Proceedings of the 35th Annual ACM Symposium on Applied Computing},
  pages={2117--2120},
  year={2020}
}

@inproceedings{wang2020assessing,
  title={Assessing Action Quality via Attentive Spatio-Temporal Convolutional Networks},
  author={Wang, Jiahao and Du, Zhengyin and Li, Annan and Wang, Yunhong},
  booktitle={Chinese Conference on Pattern Recognition and Computer Vision (PRCV)},
  pages={3--16},
  year={2020},
  organization={Springer}
}

@inproceedings{zeng2020hybrid,
  title={Hybrid Dynamic-static Context-aware Attention Network for Action Assessment in Long Videos},
  author={Zeng, Ling-An and Hong, Fa-Ting and Zheng, Wei-Shi and Yu, Qi-Zhi and Zeng, Wei and Wang, Yao-Wei and Lai, Jian-Huang},
  booktitle={Proceedings of the 28th ACM International Conference on Multimedia},
  pages={2526--2534},
  year={2020}
}

@inproceedings{jain2019unsupervised,
  title={An Unsupervised Sequence-to-Sequence Autoencoder Based Human Action Scoring Model},
  author={Jain, Hiteshi and Harit, Gaurav},
  booktitle={2019 IEEE Global Conference on Signal and Information Processing (GlobalSIP)},
  pages={1--5},
  year={2019},
  organization={IEEE}
}

@inproceedings{nekoui2020falcons,
  title={FALCONS: FAst Learner-Grader for CONtorted Poses in Sports},
  author={Nekoui, Mahdiar and Omar Tito Cruz, Fidel and Cheng, Li},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={900--901},
  year={2020}
}

@inproceedings{tang2020uncertainty,
  title={Uncertainty-aware Score Distribution Learning for Action Quality Assessment},
  author={Tang, Yansong and Ni, Zanlin and Zhou, Jiahuan and Zhang, Danyang and Lu, Jiwen and Wu, Ying and Zhou, Jie},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9839--9848},
  year={2020}
}

@inproceedings{du2020multi,
  title={Multi-Task Center-Of-Pressure Metrics Estimation from Skeleton Using Graph Convolutional Network},
  author={Du, Chen and Graham, Sarah and Jin, Shiwei and Depp, Colin and Nguyen, Truong},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={2313--2317},
  year={2020},
  organization={IEEE}
}

@inproceedings{ogata2019temporal,
  title={Temporal Distance Matrices for Squat Classification},
  author={Ogata, Ryoji and Simo-Serra, Edgar and Iizuka, Satoshi and Ishikawa, Hiroshi},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
  pages={0--0},
  year={2019}
}

@article{jain2020action,
  title={Action Quality Assessment using Siamese Network-Based Deep Metric Learning},
  author={Jain, Hiteshi and Harit, Gaurav and Sharma, Avinash},
  journal={arXiv preprint arXiv:2002.12096},
  year={2020}
}

@article{sardari2020vi,
  title={VI-Net—View-Invariant Quality of Human Movement Assessment},
  author={Sardari, Faegheh and Paiement, Adeline and Hannuna, Sion and Mirmehdi, Majid},
  journal={Sensors},
  volume={20},
  number={18},
  pages={5258},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{condorivirtual,
  title={Virtual Rehabilitation Using Sequential Learning Algorithms},
  author={Condori, Gladys Calle and Castro-Gutierrez, Eveling and Casas, Luis Alfaro}
}

@COMMENT Jaiden's refs
@misc{jaiden_1,
  title = {Chase-Riecken Musicianship Exams - Syllabi \& Study Guides},
  howpublished = {\url{https://lvmta.com/musicianship}},
  note = "[Online]"
}

@misc{jaiden_2,
  title = {The Royal Conservatory of Music-Piano-Syllabus-2015 Edition},
  howpublished = {\url{https://files.rcmusic.com//sites/default/files/files/RCM-Piano-Syllabus-2015.pdf}},
  note = "[Online]"
}

@misc{jaiden_3,
  title = {Con Brio Examinations - Grade Indications},
  howpublished = {\url{https://www.conbrioexams.com/exams-grade-inidications}},
  note = "[Online]"
}

@misc{jaiden_4,
  title = {G. Henle Verlag - Levels of difficulty (piano)},
  howpublished = {\url{https://www.henle.de/us/about-us/levels-of-difficulty-piano/}},
  note = "[Online]"
}

@misc{jaiden_5,
  title = {Las Vegas Music Teacher Association Technic - Level 10},
  howpublished = {\url{https://content.web-repository.com/s/02553545902171053/uploads/Images/Technic_Materials_10-0954933.pdf}},
  note = "[Online]"
}

@misc{hasith,
  title = {Audio Classification using Librosa and Pytorch},
  howpublished = {\url{https://medium.com/@hasithsura/audio-classification-d37a82d6715}},
  note = "[Online]"
}
